A Novel Estimator of Mutual Information for Learning to Disentangle Textual Representations

Learning disentangled representations of textual data is essential for many natural language tasks such as fair classification, style transfer and sentence generation, among others. The existent dominant approaches in the context of text data {either rely} on training an adversary (discriminator) that aims at making attribute values difficult to be inferred from the latent code {or rely on minimising variational bounds of the mutual information between latent code and the value attribute}. {However, the available methods suffer of the impossibility to provide a fine-grained control of the degree (or force) of disentanglement.} {In contrast to} {adversarial methods}, which are remarkably simple, although the adversary seems to be performing perfectly well during the training phase, after it is completed a fair amount of information about the undesired attribute still remains. This paper introduces a novel variational upper bound to the mutual information between an attribute and the latent code of an encoder. Our bound aims at controlling the approximation error via the Renyi's divergence, leading to both better disentangled representations and in particular, a precise control of the desirable degree of disentanglement {than state-of-the-art methods proposed for textual data}. Furthermore, it does not suffer from the degeneracy of other losses in multi-class scenarios. We show the superiority of this method on fair classification and on textual style transfer tasks. Additionally, we provide new insights illustrating various trade-offs in style transfer when attempting to learn disentangled representations and quality of the generated sentence.

==> additionnal_great_examples.tex <==
%%%% style transfert True
Input	0.1:	great food.
reny_1_8	0.1	great food.
reny_1_5	0.1	great food.
reny_1_3	0.1	great food.
no_reny	0.1	great food.
baseline	0.1	great food.
Input	1:	great food.
reny_1_8	1	terrible service.
reny_1_5	1	bad food.
reny_1_3	1	the worst part.
no_reny	1	bad food.
baseline	1	great food.
Input	5:	great food.
reny_1_8	5	horrible service and horrible food.
reny_1_5	5	very disappointed.
reny_1_3	5	no big deal.
no_reny	5	bad food.
baseline	5	bad service and bad food.
Input	10:	great food.
reny_1_8	10	so sad.
reny_1_5	10	the food was horrible.
reny_1_3	10	no thanks.
no_reny	10	bad food.
baseline	10	hate the place.

%%%% style transfert False


Input	0.1:	great food.
reny_1_8	0.1	great food.
reny_1_5	0.1	great food.
reny_1_3	0.1	great food.
no_reny	0.1	great food.
baseline	0.1	great food.
Input	1:	great food.
reny_1_8	1	great food.
reny_1_5	1	great food.
reny_1_3	1	great food.
no_reny	1	great food.
baseline	1	great food.
Input	5:	great food.
reny_1_8	5	great food.
reny_1_5	5	very good.
reny_1_3	5	great food.
no_reny	5	great food.
baseline	5	great service and great food.
Input	10:	great food.
reny_1_8	10	great food.
reny_1_5	10	great food.
reny_1_3	10	great service.
no_reny	10	great food.
baseline	10	love the place.
-------------------


==> propositions_modifs.tex <==
Ce qu'on fait c'est :
1. récupérer des gradients de H(X)
2. transformer la kl en renyi divergence

Pour gagner de la place se séparer de la conditionnal generation

Bien stater que Chen et al ils font cette asumption 
Le problem de CLUB c'est que c'est assez proch

Remonter la partie |Y| > 2.

En profiter pour montrer un tableau en gras.


Rajouter le biais non biaisé 

